Sim2CBF: From Forward Simulations to Implicit Control Barrier Function Safety Filtering without Model Derivatives

Failure avoidance in complex robot-environment interactions is challenging because the underlying dynamics are difficult to model accurately, and available predictive models may not provide reliable derivatives. We present Sim2CBF, a failure-avoidance framework that solves the Control Barrier Function (CBF)-Safety Filter (SF) optimization problem using only forward-model evaluations, thereby avoiding differentiation of the predictive model. Specifically, we approximate the CBF constraint using finite differences and local linear interpolation over sampled control inputs while preserving failure-avoidance guarantees. The underlying CBF is implicit and constructed from backup-policy rollouts, enabling the use of expressive predictive models such as physics-based simulators and learned world models. Compared with purely sampling-based SFs, our formulation requires fewer control samples and yields less conservative behavior than direct nominal-backup blending. We evaluate Sim2CBF in simulation, hardware box-toppling, and vision-based control tasks, demonstrating its applicability to contact-rich and learned dynamics, as well as its adaptability to changes in the predictive model.

==> glossaries.tex <==
\newacronym{cbf}{CBF}{Control Barrier Function}
\newacronym{hocbf}{HOCBF}{High-Order Control Barrier Function}
\newacronym{pcbf}{PCBF}{Policy Control Barrier Function}
\newacronym{rpcbf}{RPCBF}{Robust Policy Control Barrier Function}
\newacronym{sf}{SF}{Safety Filter}
\newacronym{nn}{NN}{Neural Network}
\newacronym{sdf}{SDF}{Signed Distance Function}
\newacronym{tbm}{TBM}{Trajectory Bundle Method}

\newacronym{qp}{QP}{Quadratic Program}
\newacronym{mpc}{MPC}{Model Predictive Control}
\newacronym{di}{DI}{Double Integrator}
\newacronym{wm}{WM}{World Model}
\newacronym{tcp}{TCP}{Tool-Center-Point}

